Building models of the Universe with hydrodynamic simulations

Hydrodynamic simulations have become irreplaceable in modern cosmology for exploring complex systems and making predictions to steer future observations. In Chapter 1, we begin with a philosophical discussion on the role of simulations in science. We argue that simulations can bridge the gap between empirical and fundamental knowledge. The validation of simulations stresses the importance of achieving a balance between trustworthiness and scepticism. Next, Chapter 2 introduces the formation of structures and comparisons between synthetic and observational data. Chapter 3 describes the production pipeline of zoom-in simulations used to model individual objects and novel methods to mitigate known shortcomings. Then, we assessed the weak scaling of the SWIFT code and found it to be one of the hydrodynamic codes with the highest parallel efficiency. In Chapter 4, we study the rotational kinetic Sunyaev-Zeldovich (rkSZ) effect for high-mass galaxy clusters from the MACSIS simulations. We find a maximum signal greater than 100 $\mu$K, 30 times stronger than early predictions from self-similar models, opening prospects for future detection. In Chapter 5, we address a tension between the distribution of entropy measured from observations and predicted by simulations of groups and clusters of galaxies. We find that most recent hydrodynamic simulations systematically over-predict the entropy profiles by up to one order of magnitude, leading to profiles that are shallower and higher than the power-law-like entropy profiles that have been observed. We discuss the dependence on different hydrodynamic and sub-grid parameters using variations of the EAGLE model. Chapter 6 explores the evolution of the profiles as a function of cosmic time. We report power-law-like entropy profiles at high redshift for both objects. However, at late times, an entropy plateau develops and alters the shape of the profile.

==> Figures/tensorsTTT.tex <==


% Gradient Info
  
\tikzset {_84j66t27s/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{89.1 bp } { -128.7 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_0afup590s}{\pgfpoint{-72bp}{104bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0.13,0.4,0.73);
rgb(400bp)=(0.13,0.4,0.73)}
\tikzset{_609aio8t5/.code = {\pgfsetadditionalshadetransform{\pgftransformshift{\pgfpoint{89.1 bp } { -128.7 bp }  }  \pgftransformscale{1.32 } }}}
\pgfdeclareradialshading{_fojkviuxj} { \pgfpoint{-72bp} {104bp}} {color(0bp)=(transparent!0);
color(0bp)=(transparent!0);
color(0bp)=(transparent!47);
color(25bp)=(transparent!17);
color(400bp)=(transparent!17)} 
\pgfdeclarefading{_b5wj3n7c1}{\tikz \fill[shading=_fojkviuxj,_609aio8t5] (0,0) rectangle (50bp,50bp); } 

% Gradient Info
  
\tikzset {_0le17zmzh/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{89.1 bp } { -128.7 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_a56sonfst}{\pgfpoint{-72bp}{104bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0.72,0.91,0.53);
rgb(400bp)=(0.72,0.91,0.53)}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,281); %set diagram left start at 0, and has height of 281

%Shape: Arc [id:dp5568348933320806] 
\draw  [draw opacity=0][line width=1.5]  (298.01,76.33) .. controls (293.96,71.56) and (228.86,86.23) .. (150.48,109.67) .. controls (70.54,133.58) and (7.07,157.55) .. (8.7,163.21) .. controls (8.7,163.22) and (8.7,163.23) .. (8.71,163.24) -- (153.44,119.93) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.95 ][line width=1.5]  (298.01,76.33) .. controls (293.96,71.56) and (228.86,86.23) .. (150.48,109.67) .. controls (70.54,133.58) and (7.07,157.55) .. (8.7,163.21) .. controls (8.7,163.22) and (8.7,163.23) .. (8.71,163.24) ;
%Shape: Ellipse [id:dp9664431763616586] 
\draw  [draw opacity=0][shading=_0afup590s,_84j66t27s,path fading= _b5wj3n7c1 ,fading transform={xshift=2}] (7.67,164.97) .. controls (-6.04,117.43) and (48.24,59.34) .. (128.91,35.21) .. controls (209.59,11.09) and (286.1,30.06) .. (299.81,77.6) .. controls (313.52,125.14) and (259.24,183.24) .. (178.57,207.36) .. controls (97.9,231.49) and (21.38,212.51) .. (7.67,164.97) -- cycle ;
%Shape: Ellipse [id:dp09658435175979996] 
\path  [shading=_a56sonfst,_0le17zmzh] (69.22,121.29) .. controls (69.22,96.49) and (107.06,76.39) .. (153.74,76.39) .. controls (200.42,76.39) and (238.26,96.49) .. (238.26,121.29) .. controls (238.26,146.08) and (200.42,166.19) .. (153.74,166.19) .. controls (107.06,166.19) and (69.22,146.08) .. (69.22,121.29) -- cycle ; % for fading 
 \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.15 ] (69.22,121.29) .. controls (69.22,96.49) and (107.06,76.39) .. (153.74,76.39) .. controls (200.42,76.39) and (238.26,96.49) .. (238.26,121.29) .. controls (238.26,146.08) and (200.42,166.19) .. (153.74,166.19) .. controls (107.06,166.19) and (69.22,146.08) .. (69.22,121.29) -- cycle ; % for border 

%Straight Lines [id:da22832575432558366] 
\draw    (153.74,121.29) -- (236.26,121.29) ;
\draw [shift={(238.26,121.29)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15277965869185528] 
\draw    (153.74,121.29) -- (153.74,78.39) ;
\draw [shift={(153.74,76.39)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp5426422111624052] 
\draw  [color={rgb, 255:red, 145; green, 191; blue, 98 }  ,draw opacity=0.57 ][line width=1.5]  (69.22,121.29) .. controls (69.22,116.77) and (107.06,113.1) .. (153.74,113.1) .. controls (200.42,113.1) and (238.26,116.77) .. (238.26,121.29) .. controls (238.26,125.81) and (200.42,129.47) .. (153.74,129.47) .. controls (107.06,129.47) and (69.22,125.81) .. (69.22,121.29) -- cycle ;
%Straight Lines [id:da6608431601210576] 
\draw [color={rgb, 255:red, 0; green, 117; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (153.65,121.37) -- (296.93,78.47) ;
\draw [shift={(299.81,77.61)}, rotate = 523.3299999999999] [color={rgb, 255:red, 0; green, 117; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da10694903518990939] 
\draw [color={rgb, 255:red, 0; green, 117; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (153.65,121.37) -- (129.73,38.1) ;
\draw [shift={(128.91,35.21)}, rotate = 433.98] [color={rgb, 255:red, 0; green, 117; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da8468146820169307] 
\draw [color={rgb, 255:red, 0; green, 117; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (153.65,121.37) -- (126.09,141.76) -- (118.78,147.17) ;
\draw [shift={(116.37,148.95)}, rotate = 323.5] [color={rgb, 255:red, 0; green, 117; blue, 255 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Arc [id:dp5594295164836465] 
\draw  [draw opacity=0][line width=1.5]  (298.06,77.44) .. controls (298.21,77.64) and (298.32,77.86) .. (298.38,78.09) .. controls (300.93,86.91) and (238.19,113.45) .. (158.26,137.36) .. controls (78.32,161.26) and (11.45,173.48) .. (8.91,164.66) .. controls (8.83,164.37) and (8.81,164.06) .. (8.87,163.73) -- (153.65,121.37) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.95 ][line width=1.5]  (298.06,77.44) .. controls (298.21,77.64) and (298.32,77.86) .. (298.38,78.09) .. controls (300.93,86.91) and (238.19,113.45) .. (158.26,137.36) .. controls (78.32,161.26) and (11.45,173.48) .. (8.91,164.66) .. controls (8.83,164.37) and (8.81,164.06) .. (8.87,163.73) ;
%Straight Lines [id:da6016249095173876] 
\draw    (153.74,121.29) -- (144.19,128.76) ;
\draw [shift={(142.61,129.99)}, rotate = 321.98] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da014393138602875943] 
\draw    (27.62,47.17) -- (54.27,47.17) ;
\draw [shift={(56.27,47.17)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da03877586066284677] 
\draw    (27.62,47.17) -- (27.62,24.27) ;
\draw [shift={(27.62,22.27)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7117917223177728] 
\draw    (27.62,47.17) -- (18.74,56.22) ;
\draw [shift={(17.33,57.65)}, rotate = 314.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (178.96,140.97) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ]  {$\mathcal{I}$};
% Text Node
\draw (55.61,185.37) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathcal{\textcolor[rgb]{0.13,0.4,0.71}{D}}$};
% Text Node
\draw (58.99,37.77) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (6.51,52.42) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (22.59,5.02) node [anchor=north west][inner sep=0.75pt]    {$z$};
% Text Node
\draw (142.44,166.1) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 0; green, 117; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{150.35684pt}\setlength\topsep{0pt}
\begin{center}
\textcolor[rgb]{0.25,0.46,0.02}{Protohalo mass distribution}
\end{center}

\end{minipage}};
% Text Node
\draw (304.54,68.62) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{a}_{\mathcal{D}}$};
% Text Node
\draw (108.93,148.8) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{b}_{\mathcal{D}}$};
% Text Node
\draw (114.71,16.94) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{c}_{\mathcal{D}}$};
% Text Node
\draw (146.26,54.62) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{c}_{\mathcal{I}}$};
% Text Node
\draw (126.17,111.74) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{b}_{\mathcal{I}}$};
% Text Node
\draw (240.52,115.33) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{a}_{\mathcal{I}}$};
% Text Node
\draw (25,219) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{151.062pt}\setlength\topsep{0pt}
\begin{center}
\textcolor[rgb]{0.2,0.27,0.71}{{\large Local gravitational potential}}
\end{center}

\end{minipage}};


\end{tikzpicture}

==> README <==
This is a University of Manchester template for a PhD thesis created by Laura Driessen (www.AstroLaura.com)

By using this template you are agreeing to check *yourself* whether it meets the requirements of the University of Manchester for PhD thesis submission. The guidelines for PhD thesis presentation can be found here: https://www.bmh.manchester.ac.uk/doctoral-academy/your-phd/thesis-submission/presentation-regulations/
I take no responsibility for the suitability of your thesis for submission.

Make sure you change everything that needs changing, like your name (must include the initial of your middle name), your supervisor's name, the colour scheme, the Declaration of Authorship, thesis title etc.

The UoM guidelines require that any blank page has the words ``Blank page'' on it, so I made a command for that. If you'd like to insert a blank page that has ``Blank page'' smack bang in the middle, just use \UoMBlankPage

The guidelines are also a bit weird about numbering, and font is important.

YOU WILL NEED TO CHANGE THE DECLARATION OF AUTHORSHIP PAGE! This is because the declarations depends on whether (and which) bits are published etc, so will vary thesis by thesis.

Not all of the preamble pages are required. You don't have to have lists of symbols, physical constants, abbreviations, popular abstract, preface etc. Read the guidelines to check which ones can be removed and what order they have to be in.

You can use fontspec to set up all the fonts, eg:
>>> \usepackage{fontspec}
>>> \setmainfont{Bitstream Vera Sans}
before \begin{document}, but then you need to go into your overleaf settings and change the LaTeX engine to XeLaTeX or LuaLaTeX. I have these lines commented out currently, and instead I'm using \usepackage{mathpazo} which is Palatino font.
You can find a list of the fonts available in overleaf (when using fontspec) here: https://www.overleaf.com/articles/fontspec-all-the-fonts/hjrpnxhrrtxc

And no, those are not the colours I used for my thesis template. I made them particularly garish so that you would choose your own colours (and there's no requirement for your thesis colours to be ugly or black and white, I checked! Colours are good!)! There are some great colour picking tools online, seriously good:
https://www.canva.com/color-palette/
https://coolors.co/
https://htmlcolorcodes.com/color-chart/
and if you need to ever convert from RGB to HEX (or vice versa):
https://www.webfx.com/web-design/hex-to-rgb/

You can make the width of the captions different by changing this line in the class file:
\captionsetup{justification=centerlast,font=small,labelfont=sc,margin=10pt}
For example, I changed mine to:
\captionsetup{justification=centerlast,font=small,labelfont={sc,bf, color=boldcolor},margin=1pt}
so that the label is bold and a colour.

Hopefully you've read all of this and checked all of the preamble for yourself to make sure it agrees with university regulations. If you haven't read all this, you might end up surprised with what your dedication says.

Good luck!  Please let me know if you come across any issues and I'll update my master template :D
